Mining Android App Usages for Generating Actionable GUI-based Execution Scenarios

GUI-based models extracted from Android app execution traces, events, or source code can be extremely useful for challenging tasks such as the generation of scenarios or test cases. However, extracting effective models can be an expensive process. Moreover, existing approaches for automatically deriving GUI-based models are not able to generate scenarios that include events which were not observed in execution (nor event) traces. In this paper, we address these and other major challenges in our novel hybrid approach, coined as MonkeyLab. Our approach is based on the Record-Mine-Generate-Validate framework, which relies on recording app usages that yield execution (event) traces, mining those event traces and generating execution scenarios using statistical language modeling, static and dynamic analyses, and validating the resulting scenarios using an interactive execution of the app on a real device. The framework aims at mining models capable of generating feasible and fully replayable (i.e., actionable) scenarios reflecting either natural user behavior or uncommon usages (e.g., corner cases) for a given app. We evaluated MONKEYLAB in a case study involving several medium-to-large open-source Android apps. Our results demonstrate that MonkeyLab is able to mine GUI-based models that can be used to generate actionable execution scenarios for both natural and unnatural sequences of events on Google Nexus 7 tablets.

==> macro.tex <==


\usepackage{amssymb}
\usepackage{ifthen}

\makeatletter

% this  is a easy way to add and highlight new text  ...
% just comment in/out the \tnew macro ..

\newcommand{\tnew}[1]{{\bf { #1 }} }
%\newcommand{\tnew}[1]{{ { #1 }} }

% math and theorem definition

\newcommand{\ndef}{\stackrel{\rm def}{=}}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\pagenumbering{arabic}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}


\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }



\newcommand\MARTY[1]{\nb{MARTY}{#1}}
\newcommand\KEVIN[1]{\nb{KEVIN}{#1}}
\newcommand\DENYS[1]{\nb{DENYS}{#1}}
\newcommand\MARIO[1]{\nb{MARIO}{#1}}
\newcommand\CARLOS[1]{\nb{CARLOS}{#1}}

\newcommand\NEW[1]{\nb{NEW}{#1}}






==> results.tex <==
\begin{table*}[tb]
\centering
\small
\caption{Summary of the Results for \emph{tasks}. Because of lack of space, results for the other AUTs are in our online appendix. }
\vspace{-0.6em}
\label{tab:results-tasks}
\begin{tabular}{lllrrrrrr|rr} \hline
Scenario&Strategy&\#TC&AVG-time(ms)&AVG-AC&AAC&AVG-MC&AMC&\#E&\#FE\\ \hline
$Testing_{EXP}$&INTERP-{\tt up}&20&35,5649.6&48.00\%&50.00\%&9.25\%&25.90\%&1,544&563\\
$Testing_{EXP}$&INTERP-{\tt down}&20&41,576.4&25.00\%&25.00\%&3.67\%&9.70\%&236&31\\
$Testing_{EXP}$&INTERP-{\tt strange}&20&57,182.55&31.25\%&50.00\%&5.04\%&16.79\%&298&64\\
$Testing_{EXP}$&BO-{\tt up}&20&576,378.15&48.75\%&50.00\%&10.17\%&24.46\%&1,854&595\\
$Testing_{EXP}$&BO-{\tt down}&20&315,663.95&50.00\%&50.00\%&10.80\%&25.76\%&1,415&443\\
$Testing_{EXP}$&BO-{\tt strange}&20&32,7096.3&50.00\%&50.00\%&11.49\%&26.34\%&1,682&512\\
$Testing_{FUNC}$&INTERP-{\tt up}&20&47,4179.1&48.75\%&75.00\%&9.88\%&34.15\%&1,933&924\\
$Testing_{FUNC}$&INTERP-{\tt down}&20&12,343.4&25.00\%&25.00\%&3.90\%&9.70\%&136&15\\
$Testing_{FUNC}$&INTERP-{\tt strange}&20&46,317.6&32.50\%&50.00\%&6.32\%&32.13\%&270&99\\
$Testing_{FUNC}$&BO-{\tt up}&17&96,2484&55.88\%&75.00\%&6.34\%&35.17\%&4,275&1,664\\
$Testing_{FUNC}$&BO-{\tt down}&17&752,156.4118&50.00\%&75.00\%&10.15\%&37.92\%&1,379&832\\
$Testing_{FUNC}$&BO-{\tt strange}&13&637,879.5385&50.00\%&75.00\%&9.11\%&35.21\%&1,232&690\\
--&DFS&--&532,923&75.00\%&75.00\%&31.19\%&31.19\%&34&34\\
--&{\tt monkey}&20&185,118.2&25.00\%&25.00\%&3.42\%&14.91\%&2,000&--\\

%Keepscore&Explore&&&&&\\
%&Functional&&&&&\\
%Tasks&Explore&&&&&\\
%&Functional&&&&&\\
%Word Web Dict.&Explore&&&&&\\
%&Functional&&&&&\\
\hline
\end{tabular}
\vspace{-0.5cm}
\end{table*}
%LMs with functional were able to find a bug, and in terms of features, were able to create several and delete tasks.
%Monkey and LM with explore data were not able (DFS?)
%Explore and Functional: display date picker in edit task activity to set task date

Table \ref{tab:results-tasks} lists the results after running all the combinations $<$$Testing,Model,Flavor,AUT$$>$ for $AUT=Tasks$; the table lists  number of \textbf{T}est \textbf{C}ases, \textbf{AV}era\textbf{G}e time for the validation and execution of a test case,  \textbf{AV}era\textbf{G}e \textbf{A}ctivity \textbf{C}overage, \textbf{A}ccumulated \textbf{A}ctivity \textbf{C}overage across the set of test cases, \textbf{AV}era\textbf{G}e \textbf{M}ethod \textbf{C}overage, \textbf{A}ccumulated \textbf{M}ethod \textbf{C}overage, number of \textbf{E}vents in the test cases, and number of \textbf{F}easible \textbf{E}vents. We use \emph{Tasks} app as a showcase to describe the findings in depth; however, for lack of space, we provide complete results for all the AUTs in the online appendix \cite{Monkeylab-OA:ICSE15}.

\subsection{\monkeylab vs. {\tt monkey} and DFS}

In this section we present the results for each AUT, and provide answers for \textbf{RQ$_1$} and \textbf{RQ$_2$}.

\subsubsection{Tasks} Using the test cases generated with the scenarios from  $Testing_{EXP}$ was enough to achieve better AAC and AMC  than {\tt monkey}, with all the {\tt BO} and {\tt INTERP}  flavors (except for {\tt INTERP}-{\tt down}). As for the test cases generated using $Testing_{FUNC}$ scenarios,  all the strategies but {\tt INTERP}-{\tt down} obtain higher AAC and AMC as compared to {\tt monkey} and DFS. Also, on average, the {\tt BO} flavors provide better coverage than {\tt INTERP}  flavors, and {\tt INTERP}-{\tt up} is the best of the interpolated flavors (in terms of achieved coverage).  Note that the number of test cases for the {\tt BO} flavors with $Testing_{FUNC}$ scenarios are less than 20. The reason for the difference is that the \emph{Chimp} hits a bug, which was injected into the AUT by the SOOT instrumentation while running the test cases generated with those strategies. Therefore, we discarded those test cases from the results to avoid any impact on the averages and the statistical tests. The main reason is that when an Android app crashes, a dialog is shown; therefore, after the crash happens, all the events in the test cases are considered as infeasible. %The crash was also detected during the systematic exploration and is manifested in a {\tt ClassCastException} with the message "android.app.TimePickerDialog cannot be cast to android.app.DatePickerDialog" in line 192 of the file {\tt org.dmfs.tasks.widget.TimeFieldEditor.java}. % After inspecting the test cases and the code, we found that \MARIO{Carlos please explain the bug}.  This is not neccesary, we injected the bug, so we do not need to report it.

\subsubsection{World Web Dictionary} Using $Testing_{EXP}$ scenario,  only {\tt INTERP-down} and {\tt INTERP-strange} method coverage outperformed {\tt monkey}; in addition {\tt INTERP-down} provided better activity coverage. When using the data collected from functional scenarios, {\tt BO-down} was the only flavor better than {\tt monkey}; and {\tt INTERP-up} was the only strategy from the interpolated family that beats {\tt monkey} in AMC. One interesting case is the fact that {\tt INTERP-down} and {\tt INTERP-strange} perform better with less data; one explanation is the fact that these flavors are more oriented to unnatural events, therefore, the larger the corpora the lower the performance of {\tt INTERP}  when the idea is to estimate the probabilities of unseen events in the sequences used for training. As compared to DFS (MC=50.57\%, AC=45.45\%), no LM-based \emph{Strategy} achieved the same result; and there is an explanation for that: initial dialog and download of required data in \emph{World Web Dictionary}. We provide a deeper explanation of this special case in Section \ref{sec:lessons}.

\subsubsection{Diabetes+} All the {\tt INTERP}  and {\tt BO} flavors (except for {\tt INTERP-down}) achieve better AAC and AMC than {\tt monkey}  using $Testing_{EXP}$ scenarios. In the case of the $Testing_{FUNC}$ scenarios, {\tt BO-strange} and {\tt INTERP-up} have larger AMC; the rest of strategies did not achieve AMC higher than {\tt monkey}; all the LM flavors outperformed the {\tt monkey} activity coverage. Conversely, DFS is the best {Strategy} in terms of AC and MC (MC=27.88\%, AC=72.73\%). Again, the low coverage of {\tt monkey} and the LM flavors is explained due to initial dialog appearing when no data is cached by the app.

\subsubsection{Keepscore} Method coverage of all {\tt INTERP}  and {\tt BO} flavors outperform {\tt monkey} with exploratory and functional data; however, {\tt monkey} provides the highest activity coverage (AVG-AC=12\%, AAC=33\%).  The coverage of our DFS implementation for \emph{Keepscore} was rather low (MC=50.57\%, AC=45.45\%), therefore, all the other strategies achieved better method and activity coverage. \emph{Keepscore} also had an initial dialog when no data/cache was kept by an AUT.

In general, the LM-based strategies implemented in \monkeylab provided better activity and method coverage as compared to {\tt monkey} in the analyzed AUTs. In terms of statistical analysis, in all the pairwise comparisons (\textit{i.e.}, {\tt monkey} vs. a \monkeylab \emph{Strategy}) with the Mann-Whitney test we found statistically significant and large differences; only in the case of {\tt monkey} vs. {\tt INTERP-strange} for $Testing_{EXP}$ scenarios there is no significant difference. Although there is significant difference of  {\tt monkey} vs. {\tt INTERP-down}, but the difference is medium. Therefore, we assert that the \textbf{ RQ$_1$ is true}.

When comparing \monkeylab to systematic exploration,  \monkeylab achieved better coverage than DFS only for \emph{Tasks} app. With the other AUTs, the LM-based strategies could not handle well initial dialogs. Therefore, our \textbf{answer to RQ$_2$ is negative}, but only in the cases of initial dialogs after clean launches; in the case of AUTs with no initial dialogs the \textbf{answer to RQ$_2$ is affirmative.}

\subsection{On Generating Test Cases with Language Models}

The Kruskall-Wallis test suggests that there is significant difference (p-value=6.79E-09) between the AAC achieved by the LM-based strategies (\textit{i.e.}, {\tt INTERP}  and {\tt BO} flavors); the result is the same for method coverage (p-value=5.70E-12). When looking into the details provided by the pairwise comparisons, there is no significant difference between the {\tt BO} flavors. However, there does exist a relevant difference between the {\tt INTERP}  flavors. When comparing {\tt INTERP}  to {\tt BO}, for method coverage there is significant difference between {\tt INTERP-down} and {\tt-up} flavors and all the {\tt BO} flavors.

The statistical tests on the results of the $Testing_{FUNC}$ scenarios confirm that the coverage achieved with the {\tt BO} flavors is similar, meanwhile the type of flavor impacts the results when using {\tt INTERP}. Also, as presented in the previous section,  {\tt INTERP} had issues when dealing with small corpora. The amount of training data impacts the ability of the {\tt INTERP}  to produce feasible events. For instance, when running the {\tt INTERP-up} and -{\tt strange} flavors for the \emph{Keepscore} app, the \emph{Test Case Generator} was not able to produce a single test case because {\tt INTERP}  was not able to adequately compute the probabilities of unseen events in the event-sequences; however those unseen events were feasible in the events vocabulary.

The {\tt BO} model was conceived to adequately estimate the probabilities of n-grams, which are not present in the training data \cite{Katz:1987}. In our context,  {\tt BO} is more suitable for generating unnatural cases than {\tt INTERP} even when the corpora is small (\textit{e.g.}, $Testing_{EXP}$ in our study). The latter operates more with events that are seen in the training data, which makes  {\tt  INTERP} more suitable for natural cases when the corpora is large. In addition, the {\tt strange} and {\tt down} flavors allow  {\tt  INTERP} to generate unnatural test cases, but again, a larger corpora is required for {\tt  INTERP} to generate meaningful test cases.


\subsection{Learned Lessons}
\label{sec:lessons}

Automated GUI testing in Android apps should take into account the following information this Empirical has shown can pose issues for various testing \emph{Strategies}.

\textbf{Encapsulated components}.  First, encapsulated components\footnote{An encapsulated component is the one where all the rendering and events handling is managed directly by the component.} (\textit{e.g.}, {\tt KeyboardView}, {\tt AutoCompleteTextView}, {\tt CalendarView, Date Picker}) can not be analyzed during systematic exploration, because the sub-components (\textit{e.g.}, each key of the keyboard) are not available for ripping at execution time;  thus, the sub-components are not recognized by the {\tt View Server} or the {\tt Hierarchy Viewer}. This type of components require a predefined model of the feasible events with the locations and areas of these sub-components.

\textbf{Clean and dirty launches}. Automated test cases, and their generation need to be oriented both for clean (\textit{i.e.}, no previous data or cache in the app) and dirty launches (\textit{i.e.},  the app keeps data from previous executions). In case of a clean launch initial dialogs, and the initial download mechanism for apps requiring content from external providers (\textit{e.g.}, dictionaries that download the database during the first launch) may cause problems. The former (initial dialog) was an issue for the {\tt monkey} tool and our LM-based strategies, because initial dialogs prevented the {\tt monkey}  and our \emph{Chimp} from testing the other screens. A database initialization spalshscreen affected for \emph{World Web Dictionary}. After this initial dialog in \emph{World Web Dictionary}, the required data is downloaded by the AUT. \monkeylab does not learn the idle times between events from the collected traces, so the \emph{Chimp} executes the events without  inter-arrival time considerations. Therefore, the \emph{Chimp} does not wait while the data is being downloaded, and  starts to execute events from the test cases; although some events are valid in the test case, some of them are declared as infeasible during the "downloading" process in the AUT. This was also an issue for {\tt monkey}, which tried to execute GUI events during the "downloading" process. For the DFS-based exploration, to avoid the issue, we had to hardcode a waiting time right after the initial dialog (which explains higher coverage numbers for DFS). 

\textbf{Inter-arrival time for events.} The arrival time between events, during real execution of mobile apps, should also be modeled to reduce idle time during testing and to avoid the situation where feasible events become unfeasible (\textit{e.g.}, because of early execution). In our experiments we assumed inter-arrival time for {\tt monkey} to be 1000ms because the AUTs in our study do not access dynamic content from external providers (except for the case of data downloading in \emph{World Web Dictionary}) . In the case of DFS and \monkeylab  no inter-arrival  time definition was required because of the time of the ripping steps and the time required to get the info from the {\tt View Server}. However, probability distributions of inter-arrival time could be learned from real executions, which is a subject of our future work.

\textbf{Training corpus size}. The last lesson gleaned from this study is the fact that, in order to be effective as a test generation tool, the training corpus for the LMs must be robust when leveraging interpolated n-grams.  This is observed in most of the the test cases for the AUTs (mostly for \emph{Keepscore}) for which the  LM-based strategies were not able to produce a response. Which suggests that when small corpora is available, it is better to use {\tt BO} flavors.

==> threats.tex <==
The data collection during the {\tt \textit{Record}} phase was done by external participants (none of the authors was involved) to avoid any type of bias. However, a threat to the \emph{interval validity} are the scenarios (events) that the participants executed during the exploratory and functional testing. These events were used to train the LMs, therefore, the quality of the training data directly impacts the results. To reduce this threat, we asked the participants to start every execution from scratch (i.e., by clearing app data/cache) and to go back to the app once the execution is transferred to another app. A further threat to \emph{internal validity} concerns the non-deterministic nature of the LMs, consequently, we do not report coverage of individual scenarios; the coverage computation is accumulated iteratively for each strategy over 100 corresponding actionable scenarios.  

%of decompilation in the source code measurements. For instance, the amount of total methods in a AUT is extracted from the source code by using AST (Abstract Syntax Tree) exploration. Those values are used to compute the $AC$ and $MC$ of the experiments. We found that the Procyon decompiler was not able to decompile few classes.  Therefore, the total number of methods extracted from decompiled code could be not exactly the same than in the source code of the app (unfortunately not all the AUTs in the study are open source). To reduce the impact of this issue, we computed the total number of methods from the source code, when available, otherwise we used the decompiled code. %(Feedly, Word Web Dictionary, and Diabetes+). 
%Also, in addition to the coverage, we reported the covered methods or activities, which computation is not impacted by the decompilation issue. 
%A further threat to \emph{internal validity} concerns the non-deterministic nature of the LMs, consequently, we do not report coverage of individual scenarios; the coverage computation is averaged for each strategy over the 20 corresponding actionable scenarios.   
A  threat to \emph{external validity} is the number of apps used in the study. We are not claiming that these results will necessarily generalize to all theAndroid apps. However, we used medium-to-large apps (size) that implement frequently used features (i.e., budget, tasks, and fuel consumption management). Finally, our results should not be generalized to all the mobile platforms, neither to all the categories of Android apps. Therefore, a larger study with a representative sample of mobile apps should be executed to warrant generalizability of the results.
